SOCRATES: Towards a Unified Platform for Neural Network Analysis

Studies show that neural networks, not unlike traditional programs, are subject to bugs, e.g., adversarial samples that cause classification errors and discriminatory instances that demonstrate the lack of fairness. Given that neural networks are increasingly applied in critical applications (e.g., self-driving cars, face recognition systems and personal credit rating systems), it is desirable that systematic methods are developed to analyze (e.g., test or verify) neural networks against desirable properties. Recently, a number of approaches have been developed for analyzing neural networks. These efforts are however scattered (i.e., each approach tackles some restricted classes of neural networks against certain particular properties), incomparable (i.e., each approach has its own assumptions and input format) and thus hard to apply, reuse or extend. In this project, we aim to build a unified framework for developing techniques to analyze neural networks. Towards this goal, we develop a platform called SOCRATES which supports a standardized format for a variety of neural network models, an assertion language for property specification as well as multiple neural network analysis algorithms including two novel ones for falsifying and probabilistic verification of neural network models. SOCRATES is extensible and thus existing approaches can be easily integrated. Experiment results show that our platform can handle a wide range of networks models and properties. More importantly, it provides a platform for synergistic research on neural network analysis.

==> discussion.tex <==
\section{Discussions}


\subsection{Soundness}
In most machine learning tasks, input data needs to be pre-processed before feeding into a learning model, while the pre-processing step may introducing precision loss sometimes. For example, such imprecision may occur when we normalize the image data (e.g. $pixel\_value/255.0$) before feeding them into an image recognition model. When solving a network against a given property (defined by the assertion language), such pre-processing step may affect the soundness of our approach. 

The root cause of this problem is that, the pre-processing function $f:x \to x_{in}$ is not usually a bijective mapping for \emph{natural range} over $x$ and $x_{in}$. 
A naive way to address this problem is to check the result after solving and try to fetch another solution if the result is not sound. In this approach, we take a different method, encoding the pre-processing step into the objective function for optimisation.
% (We may need to explain more if we want to discuss this problem. I create the notation \{natural range\} (NR for short) here. For example, for image recognition tasks, $NR(x) = \{n^m| n \in N, n>=0, n<=255, m=784 ~(i.e.~dim)\}$, and $NR(x_{in}) = \{f^m| f \in FP_{64}, f>=0.0, f <= 1.0, m=784\}$).

% \todo{We address such problem via validating the result???}



Usually the pre-processing function is simple in the real domain and its inverse is easy to obtain. Thus, we assume a pre-processing function $f: x \to x_{in}$ and its inverse $f^{-1}: x_{in} \to x$ are given. We should note that, function $f$ and $f^{-1}$ are mutually inverse on the real domain. For example, if $f(x)= x/255.0$, then $f^{-1}(x_{in}) = x_{in} * 255.0$. However, in the application domains represented in digital computers such as machine integer and floating points, they are usually not precisely inverse, which is also the root cause of the soundness issue. In other words, in the computational domains (\todo{what are official names for such domains}), $f(f^{-1}(x_{in}))=x_{in}$ and $f^{-1}(f(x))=x$ does not hold all the time.

Given a neural network $model(x_{in}) = y$, we define another similar model $model^{\star}$ to mimic its behavior as well as considering the soundness issues. The model is defined as $model^{\star}(x_{in}) = model(f(f^{-1}(x_{in})))$. With this model, we can encode the network into the objective function.

One issue with such encoding is, it might not render the whole objective function as smooth as before. (Although the numerical function is non-smooth in the floating point domain). To overcome this issue, we add an extra penalty item to the objective function. $penalty(x_{in}) = (x_{in} - f(f^{-1}(x_{in})))^2$.

In one word, to resolve the soundness issues, we replace all the $model(x_{in})$ evaluation in the objective function with $model^{\star}(x_{in}) + penalty(x_{in})$.


\subsection{Design Choices}

\noindent\textbf{Layer-based Representation}
In essence, a neural network is a computation graph, which propagates inputs with defined computation to establish the desired outputs. Neural networks can be in many forms, but the most popular network models are usually composed layer-by-layer. Therefore, in this paper, we assume the neural network is represented as a layer-based model which greatly simplifies the network representation while sacrifices a little flexibility. 

To support more customized neural networks, we may break the layer-based representation into fine-grained representation, like operations defined by TensorFlow framework. \todo{We would leave such extension to nSolver for future work.}

\bigskip
\noindent\textbf{Json format}
From my understanding, our json format is more like an intermediate representation for neural networks. If we use .json format as the input, \todo{we may need to justify why json is a good representation. What is the real advantage of using json format?}

\bigskip
\noindent\textbf{System Architecture} \todo{Let's leave it here for now}
We assume json format is very suitable for the problem for now. From a system perspective, how would the following system design sounds?

\noindent\emph{nSolver} is a system composing of three parts, a front-end, a mid-end, and a back-end.

\begin{itemize}
\item The front-end 
\begin{itemize}
\item [-] takes a network in a variety number of formats, such as .tf, .pt, etc., and converts them into the .json format; 
\item [-] takes a property in some formats and convert it into the assertion language.
\end{itemize}

\item The mid-end manipulates the .json model and the assertion language for better optimization, and yields an objective function.

\item The back-end adapts optimization techniques and solve the objective function passed from the mid-end. It outputs the solving results.

% \item To guarantee the soundness of our approach, we may develop a component to validate the solving result.
\end{itemize}



==> evaluation.tex <==
\subsection{Evaluation} \label{evaluatoin}

\noindent \emph{Effectiveness} Next, we compare \name with existing tools in terms of effectiveness, i.e., whether a property can be effectively verified or falsified. Note that \name integrates existing verifiers such as Deeppoly (thanks to \name's extensibility). To be fair, only the two verification engines described in Section~\ref{engines} are applied in the experiments. \sj{Add computer configuration here. Accidentally removed the sentence :-(}

We collect a set of neuron networks and adversarial properties in the literature, including \sj{this is good, just wondering whether we can systematically collect all the example in all these papers and claim that we build a repository of benchmark, like the one from SVCOMP}:
\begin{itemize}
    \item 45 fully-connected networks and 10 properties used in the experiments of Reluplex.
    \item 21 fully-connected and convolutional networks and local robustness property with 100 samples from 2 datasets used in the experiments of DeepPoly and DeepZono.
    \item 3 fully-connected networks and local robustness property in fairness conditions with 100 samples from 3 datasets used in the experiments of ADF.
    \item 4 recurrent networks and local robustness property with 10 samples from 2 datasets in XXX.
    \item 1 convolutional network and local robustness property with 10000 samples in MNIST challenge.
\end{itemize}

The results of the first experiment with 10 properties and 45 networks reported in Reluplex paper are shown in Table~\ref{reluplex}.
The first column show the IDs of the properties. The second column shows the number of network is checked with each property. The last two columns show the results of Reluplex and \name respectively. Regretfully, within $1$ hour, Reluplex cannot finish any experiment and give all timeout results. The results of \name are divided into SAT sub-column (which shows the number of networks that \name can find the sample satisfies adversarial properties) and Probably UNSAT sub-column (which shows the number of networks that \name failed to find adversarial samples). To validate the \name results, we compare them with the results reported in Reluplex paper (which is run in a lot more time). The comparison shows that \name results are consistent with reported Reluplex results, except for the Property $2$ where Reluplex can find $6$ more SAT samples, and Property $8$ where Reluplex can find $1$ more SAT sample.

% \begin{table}[t]
% \begin{center}
% \begin{tabular}{| c | c | c | c | c | c | c |}
% \hline
%  \multirow{2}{*}{Property} & \multirow{2}{*}{Network} &
%  \multicolumn{2}{c|}{Reluplex} & \multicolumn{3}{c|}{\name} \\
%  \cline{3-7}
%  & & Res & Time & SAT & PUNSAT & Time \\
%  \hline
%  1 & 45 & TO & - & 0 & 45 & 28.28s \\
%  2 & 36 & TO & - & 29 & 7 & 21.99s \\
%  3 & 42 & TO & - & 0 & 42 & 26.48s \\
%  4 & 42 & TO & - & 0 & 42 & 25.44s \\
%  5 & 1 & TO & - & 0 & 1 & 0.60s \\
%  6 & 1 & TO & - & 0 & 1 & 1.25s \\
%  7 & 1 & TO & - & 0 & 1 & 1.21s \\
%  8 & 1 & TO & - & 0 & 1 & 0.61s \\
%  9 & 1 & TO & - & 0 & 1 & 0.58s \\
%  10 & 1 & TO & - & 0 & 1 & 0.57s \\
%  \hline
% \end{tabular}
% \caption{Experiment with Reluplex. Timeout: 1 hour for 10 properties}
% \label{reluplex}
% \end{center}
% \end{table}

For the second experiment, we use $13$ network structures reported in DeepPoly paper. We notice that some network structures have defended and undefended versions and so in total, we have $21$ networks. The experiment is to check the local robustness property around 100 original sample from MNIST and CIFAR-$10$ datasets. The results of this experiment are shown in Table~\ref{deeppoly}. In the table, the first column shows the name of the network. The second column show the number of correctly classified original samples over the set of $100$ samples. We notice that all $3$ tools DeepPoly, DeepZono, and \name only perform the analysis on  correctly classified samples. The next $3$ columns show the results of DeepPoly, DeepZono, and \name respectively. In this experiment, we use infinity-norm distance with $0.1$ and $0.5$ are the values of the distance. We notice the duality between the results of DeepPoly and DeepZono compare to \name. In DeepPoly and DeepZono, they try to prove a sample is safe, which means there is no adversarial sample in a pre-defined distance. On the other hand, \name try to find the adversarial samples as closed as possible to the original samples. Because of that, the values in sub-columns $0.1$ and $0.5$ of DeepPoly and DeepZono show the number of safe samples, while for \name, they show the number of found adversarial samples. From the table, we see that \name finds less adversarial samples in distance $0.1$ than in distance $0.5$. At the same time, DeepPoly and DeepZono prove more safe samples in distance $0.1$ than in distance $0.5$. It shows the consistency between these tools, which helps to validate the results of \name.

\begin{table*}[t]
\begin{center}
\setlength{\tabcolsep}{3.8pt}
\begin{tabular}{| l | c | c | c | c | c | c | c | c | c | c | c | c |}
\hline
 \multirow{2}{*}{Network} & \multirow{2}{*}{Valid Points} & \multicolumn{4}{c|}{DeepPoly} & \multicolumn{4}{c|}{DeepZono} & \multicolumn{3}{c|}{\name} \\
 \cline{3-13}
 & & 0.1 & Time & 0.5 & Time & 0.1 & Time & 0.5 & Time & 0.1 & 0.5 & Time \\
 \hline
 MNIST\_ReLU\_4\_1024 & 98 & TO & - & TO & - & TO & - & TO & - & 1 & 93 & 4m23.45s \\
 MNIST\_ReLU\_6\_100 & 99 & 0 & 0m25.34s & 0 & 0m18.42s & 0 & 8m37.52s & 0 & 8m25.39s & 9 & 98 & 2m17.94s \\
 MNIST\_ReLU\_9\_200 & 97 & 0 & 3m15.62s & 0 & 2m17.43s & TO & - & TO & - & 8 & 97 & 3m19.60s \\
 MNIST\_Sigmoid\_6\_500 & 95 & TO & - & TO & - & TO & - & TO & - & 54 & 95 & 5m5.75s \\
 MNIST\_Sigmoid\_6\_500\_PGD\_0.1 & 100 & TO & - & TO & - & TO & - & TO & - & 3 & 88 & 4m37.68s \\
 MNIST\_Sigmoid\_6\_500\_PGD\_0.3 & 97 & TO & - & TO & - & TO & - & TO & - & 5 & 44 & 4m45.00s \\
 MNIST\_Tanh\_6\_500 & 99 & TO & - & TO & - & TO & - & TO & - & 9 & 81 & 4m19.17s \\
 MNIST\_Tanh\_6\_500\_PGD\_0.1 & 100 & TO & - & TO & - & TO & - & TO & - & 2 & 80 & 4m17.19s \\
 MNIST\_Tanh\_6\_500\_PGD\_0.3 & 100 & TO & - & TO & - & TO & - & TO & - & 1 & 28 & 4m52.39s \\
 MNIST\_Conv\_Small\_ReLU & 100 & 45 & 1m3.27s & 0 & 1m6.13s & 35 & 8m12.10s & 0 & 17m14.64s & 4 & 89 & 3m56.46s \\
 MNIST\_Conv\_Small\_ReLU\_DiffAI & 99 & 95 & 0m38.18s & 0 & 0m59.41s & 94 & 5m9.41s & 0 & 10m27.17s & 2 & 27 & 4m9.53s \\
 MNIST\_Conv\_Small\_ReLU\_PGD & 100 & 86 & 1m4.71s & 0 & 1m16.57s & 76 & 8m52.38s & 0 & 18m18.17s & 0 & 32 & 3m17.60s \\
 MNIST\_Conv\_Big\_ReLU\_DiffAI & 95 & TO & - & TO & - & 92 & 49m37.48s & TO & - & 0 & 16 & 45m53.35s \\
 MNIST\_Conv\_Super\_ReLU\_DiffAI & 99 & TO & - & TO & - & TO & - & TO & - & 1 & 19 & 104m53.03s \\
 CIFAR\_ReLU\_6\_100 & 16 & 0 & 0m16.89s & 0 & 0m16.33s & 0 & 14m12.94s & 0 & 10m15.30s & 3 & 3 & 0m37.51s \\
 CIFAR\_ReLU\_7\_1024 & 16 & TO & - & TO & - & TO & - & TO & - & 4 & 4 & 2m53.01s \\
 CIFAR\_ReLU\_9\_200 & 9 & 0 & 1m16.51s & 0 & 0m50.50s & TO & - & 0 & 23m16.77s & 1 & 1 & 0m29.51s \\
 CIFAR\_Conv\_Small\_ReLU & 59 & 0 & 1m51.90s & 0 & 1m42.57s & TO & - & TO & - & 58 & 59 & 9m31.84s \\
 CIFAR\_Conv\_Small\_ReLU\_DiffAI & 53 & 0 & 0m59.15s & 0 & 1m14.79s & 0 & 20m5.86s & TO & - & 31 & 53 & 2m11.53s \\
 CIFAR\_Conv\_Small\_ReLU\_PGD & 70 & 0 & 2m4.52s & 0 & 1m54.91s & TO & - & TO & - & 59 & 70 & 3m38.65s \\
 CIFAR\_Conv\_Big\_ReLU\_DiffAI & 60 & TO & - & TO & - & TO & - & TO & - & 52 & 60 & 15m49.98s \\
 \hline
\end{tabular}
\caption{Experiment with DeepPoly and DeepZono. Timeout: small networks (30 mins), big networks (1 hour), super networks (2 hours)}
\label{deeppoly}
\end{center}
\end{table*}

For the third experiment, we use $3$ fully-connected neuron networks trained with $3$ different datasets used in ADF paper. We do not compare directly with ADF because ADF try to generate as many adversarial samples as possible while \name only try to generate one. Moreover, ADF finds adversarial samples in integer domain while \name works in floating-point domain. Because of that, in this experiment, we randomly choose $100$ samples in the datasets and try to perform untargeted local robustness attack with fairness constraints on them. The protected features are the same as in ADF paper. The result is showns in Table~\ref{adf}. In the table, the first column shows the name of the network, the second column show the number of correctly classified samples, and the third columns show the number of generated adversarial samples. From the table, we see that from $3$ datasets, \name can generate adversarial samples for 10\%, 40\%, and 45\% of original samples respectively.

\begin{table}[t]
\begin{center}
\setlength{\tabcolsep}{10pt}
\begin{tabular}{| l | c | c | c |}
\hline
 Network & Valid Points & Result & Time \\
 \hline
 Bank & 99 & 10 & 20.24s \\
 Census & 86 & 34 & 27.79s \\
 Credit & 100 & 45 & 31.52s \\
 \hline
\end{tabular}
\caption{Experiment with ADF. Timeout: 5 minutes for each network.}
\label{adf}
\end{center}
\end{table}

In the forth experiment, we try to generate adversarial samples for recurrent neuron networks. To the best of our knowledge, we are the first to perform this kind of experiment. We choose $2$ LSTM and GRU networks trained with $2$ dataset Jigsaw and Wiki from XXX as the test subjects. For each network, we randomly choose $10$ samples from the test set and perform untargeted local robustness attack on them. The result is shown in Table~\ref{rnn}, with the meaning of each column is the same as in Table~\ref{adf}. From the table, we see that \name can generate adversarial samples for 100\% of original samples.

\begin{table}[t]
\begin{center}
\begin{tabular}{| l | c | c | c |}
\hline
 Network & Valid Points & Result & Time \\
 \hline
 Jigsaw\_GRU & 9 & 9 & 38m14.25s \\
 Jigsaw\_LSTM & 10 & 10 & 26m48.62s \\
 Wiki\_GRU & 10 & 10 & 26m36.41s \\
 Wiki\_LSTM & 10 & 10 & 39m13.57s \\
 \hline
\end{tabular}
\caption{Experiment with RNN. Timeout: 1 hour for each network.}
\label{rnn}
\end{center}
\end{table}

Finally, we notice that unlike other specific tools, \name is a generate tool used to check a wide range of properties for a wide range of neuron networks. Because of that, other tools may have some optimizations for specific problems which outperform the general approach in \name. For instance, ADF has heuristic to choose the initial samples in their global robustness attack. We also perform the experiment with MNIST challenge and see that the result of \name is far less than other adversarial samples generation tools (e.g., C\&W). These results are indeed expected and we have plans to improve the performance of \name for each specific problem in the future.\\

\begin{table}[t]
\begin{center}
\begin{tabular}{| c | c | c | c | c |}
\hline
 \multirow{2}{*}{Property} & \multirow{2}{*}{Network} &
 \multicolumn{3}{c|}{\name} \\
 \cline{3-5}
 &  & H0 & H1 & Time \\
 \hline
 1 & 45 & 45 & 0 & 37.62s \\
 2 & 36 & 14 & 22 & 30.64s \\
 3 & 42 & 42 & 0 & 34.79s \\
 4 & 42 & 42 & 0 & 34.85s \\
 5 & 1 & 1 & 0 & 0.83s \\
 6 & 1 & 1 & 0 & 1.67s \\
 7 & 1 & 1 & 0 & 0.88s \\
 8 & 1 & 1 & 0 & 0.83s \\
 9 & 1 & 1 & 0 & 0.84s \\
 10 & 1 & 1 & 0 & 0.83s \\
 \hline
\end{tabular}
\caption{Experiment with Reluplex and SPRT. Timeout: 1 hour for 10 properties}
\label{reluplex-sprt}
\end{center}
\end{table}

\begin{table*}[t]
\begin{center}
\setlength{\tabcolsep}{3.8pt}
\begin{tabular}{| l | c | c | c | c | c | c | c |}
\hline
 \multirow{2}{*}{Network} & \multirow{2}{*}{Valid Points} & \multicolumn{3}{c|}{\name 0.1} & \multicolumn{3}{c|}{\name 0.5} \\
 \cline{3-8}
 & & H0 & H1 & Time & H0 & H1 & Time \\
 \hline
 MNIST\_ReLU\_4\_1024 & 98 & 95 & 3 & 0m42.35s & 34 & 64 & 0m32.15s \\
 MNIST\_ReLU\_6\_100 & 99 & 99 & 0 & 0m5.73s & 11 & 88 & 0m2.58s \\
 MNIST\_ReLU\_9\_200 & 97 & 90 & 7 & 0m10.40s & 6 & 91 & 0m5.12s \\
 MNIST\_Sigmoid\_6\_500 & 95 & 92 & 3 & 0m38.78s & 10 & 85 & 0m16.49s \\
 MNIST\_Sigmoid\_6\_500\_PGD\_0.1 & 100 & 98 & 2 & 0m38.30s & 43 & 57 & 0m22.23s \\
 MNIST\_Sigmoid\_6\_500\_PGD\_0.3 & 97 & 96 & 1 & 0m35.12s & 69 & 28 & 0m23.79s \\
 MNIST\_Tanh\_6\_500 & 99 & 97 & 2 & 0m34.12s & 7 & 92 & 0m15.54s \\
 MNIST\_Tanh\_6\_500\_PGD\_0.1 & 100 & 100 & 0 & 0m33.62s & 38 & 62 & 0m21.29s \\
 MNIST\_Tanh\_6\_500\_PGD\_0.3 & 100 & 99 & 1 & 0m36.28s & 87 & 13 & 0m24.93s \\
 MNIST\_Conv\_Small\_ReLU & 100 & 99 & 1 & 0m22.16s & 63 & 37 & 0m16.60s \\
 MNIST\_Conv\_Small\_ReLU\_DiffAI & 99 & 99 & 0 & 0m20.07s & 9 & 90 & 0m4.23s \\
 MNIST\_Conv\_Small\_ReLU\_PGD & 100 & 100 & 0 & 0m21.40s & 27 & 73 & 0m9.21s \\
 MNIST\_Conv\_Big\_ReLU\_DiffAI & 95 & 95 & 0 & 2m23.19s & 0 & 95 & 0m19.16s \\
 MNIST\_Conv\_Super\_ReLU\_DiffAI & 99 & 98 & 1 & 7m42.59s & 0 & 99 & 2m12.77s \\
 CIFAR\_ReLU\_6\_100 & 16 & 7 & 9 & 0m7.82s & 0 & 16 & 0m6.03s \\
 CIFAR\_ReLU\_7\_1024 & 16 & 8 & 8 & 1m13.75s & 0 & 16 & 1m9.70s \\
 CIFAR\_ReLU\_9\_200 & 9 & 5 & 4 & 0m11.11s & 0 & 9 & 0m10.61s \\
 CIFAR\_Conv\_Small\_ReLU & 59 & 45 & 14 & 0m16.38s & 0 & 59 & 0m4.36s \\
 CIFAR\_Conv\_Small\_ReLU\_DiffAI & 53 & 46 & 7 & 0m14.38s & 12 & 41 & 0m7.26s \\
 CIFAR\_Conv\_Small\_ReLU\_PGD & 70 & 61 & 9 & 0m17.72s & 12 & 58 & 0m8.88s \\
 CIFAR\_Conv\_Big\_ReLU\_DiffAI & 60 & 47 & 13 & 1m47.60s & 0 & 60 & 0m27.22s \\
 \hline
\end{tabular}
\caption{Experiment with DeepPoly and DeepZono and SPRT. Timeout: small networks (30 mins), big networks (1 hour), super networks (2 hours)}
\label{deeppoly-sprt}
\end{center}
\end{table*}

\begin{table}[t]
\begin{center}
\setlength{\tabcolsep}{10pt}
\begin{tabular}{| l | c | c | c | c |}
\hline
 Network & Valid Points & H0 & H1 & Time \\
 \hline
 Bank & 99 & 87 & 12 & 2.19s \\
 Census & 86 & 46 & 40 & 1.79s \\
 Credit & 100 & 54 & 46 & 1.95s \\
 \hline
\end{tabular}
\caption{Experiment with ADF and SPRT. Timeout: 5 minutes for each network.}
\label{adf-sprt}
\end{center}
\end{table}

\begin{table*}[t]
\begin{center}
\begin{tabular}{| l | c | c | c | c | c | c | c |}
\hline
 \multirow{2}{*}{Network} & \multirow{2}{*}{Valid Points} & \multicolumn{3}{c|}{\name 0.1} & \multicolumn{3}{c|}{\name 0.5} \\
 \cline{3-8}
 & & H0 & H1 & Time & H0 & H1 & Time \\
 \hline
 Jigsaw\_GRU & 9 & 10 & 0 & 24.66s & 8 & 1 & 24.85s \\
 Jigsaw\_LSTM & 10 & 10 & 0 & 28.68s & 8 & 2 & 30.94s \\
 Wiki\_GRU & 10 & 10 & 0 & 39.78s & 9 & 1 & 38.66s \\
 Wiki\_LSTM & 10 & 10 & 0 & 42.38s & 7 & 3 & 45.44s \\
 \hline
\end{tabular}
\caption{Experiment with RNN and SPRT. Timeout: 1 hour for each network.}
\label{rnn-sprt}
\end{center}
\end{table*}

\noindent
\emph{RQ3: Can \name generate adversarial samples efficiently?}

To answer this question, we measure the time needed to run the experiment with \name and compare it with other tools when possible. The results are shown in columns \emph{Time} of Tables~\ref{reluplex},~\ref{deeppoly},~\ref{adf}, and~\ref{rnn}. We notice than because \name try to generate adversarial samples as closed to original samples as possible, we only need to run \name once in the experiment with DeepPoly and DeepZono, and so \name only has $1$ column \emph{Time} instead of $2$ as the other tools.

From Tables~\ref{reluplex} and \ref{deeppoly}, we see that \name run much faster than Reluplex, DeppPoly, and DeepZono. While those $3$ tools show a lot of timeout results, \name can finish all the analysis tasks on time. In Table~\ref{adf}, again we see \name can generate a hundred of adversarial samples in less than 30s. In Table~\ref{rnn}, due to the complexity of recurrent networks and their samples, \name needs more time to complete but in average, it only takes less than 5 minutes for an adversarial sample. With these results, we conclude that \name is efficient enough to be used in real application.

